Propagators and Solvers for the Algebra of Modular Systems

To appear in the proceedings of LPAR 21. Solving complex problems can involve non-trivial combinations of distinct knowledge bases and problem solvers. The Algebra of Modular Systems is a knowledge representation framework that provides a method for formally specifying such systems in purely semantic terms. Formally, an expression of the algebra defines a class of structures. Many expressive formalism used in practice solve the model expansion task, where a structure is given on the input and an expansion of this structure in the defined class of structures is searched (this practice overcomes the common undecidability problem for expressive logics). In this paper, we construct a solver for the model expansion task for a complex modular systems from an expression in the algebra and black-box propagators or solvers for the primitive modules. To this end, we define a general notion of propagators equipped with an explanation mechanism, an extension of the alge- bra to propagators, and a lazy conflict-driven learning algorithm. The result is a framework for seamlessly combining solving technology from different domains to produce a solver for a combined system.

==> idp-latex/idp-latex-no-theorem.tex <==
%IMPORTANT: ONLY INCLUDE AS \input{idp-latex/idp-latex-no-theorem}
\usepackage{import}

\subimport{idp-latex/}{includes-no-theorems}
\subimport{idp-latex/}{common-citations}




%The following are directives for LaTeX editors that collect ``included files'' to autocomplete macros etcetera
\ignore{
\include{includes-no-theorems}
\include{common-citations}
}

==> idp-latex/idp-listings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             Stuff for writing IDP source code with coloring              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\usepackage[final]{listings}

	\lstdefinelanguage{idp}{
		morekeywords=[1]{query(}, %to ignore procedure calls to query
		morekeywords=[2]{namespace,vocabulary,theory,structure,procedure,term,set,formula, spec, specification,query},
		morekeywords=[3]{include,using,type,isa,contains,partial,extern,LFD,GFD,constructed,from,constraint,pred,supertype,of,subtype,define},
		morekeywords=[4]{int,float,char,string,nat},
		morekeywords=[5]{if,then,else,for,end},
		morecomment=[s]{/*}{*/},	
		morecomment=[l]{//}
	}
	\lstset{
		language=idp,
		tabsize=3,
		basicstyle=\small,
		frame=none,
		frame=single,
		showstringspaces=false,
		breaklines = true,
		alsoletter=(,
		commentstyle=\commentstyle,
		keywordstyle=[1],
		keywordstyle=[2]\color{BrickRed}\bfseries,
		keywordstyle=[3]\color{OliveGreen}\bfseries,
		keywordstyle=[4]\color{Blue}\bfseries,
		keywordstyle=[5]\color{Violet}\bfseries,
		literate={~} {$\sim$}{1}
	}
	\newcommand{\code}[1]{\texttt{#1}}

